Approximating dynamical correlation functions with constant depth quantum circuits

One of the most important quantities characterizing the microscopic properties of quantum systems are dynamical correlation functions. These correlations are obtained by time-evolving a perturbation of an eigenstate of the system, typically the ground state. In this work, we study approximations of these correlation functions that do not require time dynamics. We show that having access to a circuit that prepares an eigenstate of the Hamiltonian, it is possible to approximate the dynamical correlation functions up to exponential accuracy in the complex frequency domain $\omega=\Re(\omega)+i\Im(\omega)$, on a strip above the real line $\Im(\omega)=0$. We achieve this by exploiting the continued fraction representation of the dynamical correlation functions as functions of frequency $\omega$, where the level $k$ approximant can be obtained by measuring a weight $O(k)$ operator on the eigenstate of interest. In the complex $\omega$ plane, we show how this approach allows to determine approximations to correlation functions with accuracy that increases exponentially with $k$. We analyse two algorithms to generate the continuous fraction representation in scalar or matrix form, starting from either one or many initial operators. We prove that these algorithms generate an exponentially accurate approximation of the dynamical correlation functions on a region sufficiently far away from the real frequency axis. We present numerical evidence of these theoretical results through simulations of small lattice systems. We comment on the stability of these algorithms with respect to sampling noise in the context of quantum simulation using quantum computers.

==> preamble.tex <==
%%%%%%%%%%%%%%%
%% Keep useful packages here that will be wanted in most projects 
%% Add less common packages on a per-project basis
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
%% Defaults
%%%%%%%%%%%%%%%
\usepackage[a4paper, total={7in, 9in}]{geometry}
\usepackage[utf8]{inputenc}
\usepackage{tikz}
\usepackage{background}
\usepackage{caption}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage[normalem]{ulem}
\usepackage{quantikz}

\usepackage{amsthm}

\usepackage{longtable}


\newcommand{\ES}[1]{{\color{magenta} ES: #1}}

\backgroundsetup{
   scale=1,
   angle=0,
   opacity=1,
   color=black,
   contents={\begin{tikzpicture}[remember picture, overlay, font=\sffamily]
      \node at ([xshift=-3cm,yshift=-1.5cm] current page.north east)
            {\includegraphics[width = 5cm]{Phasecraft-HorizontalLogo.pdf}};
     \node at ([xshift=6cm,yshift=-1.5cm] current page.north west)
            {DRAFT: CONFIDENTIAL, DO NOT CIRCULATE FURTHER};
     \end{tikzpicture}}
 }

% \backgroundsetup{
%    scale=1,
%    angle=0,
%    opacity=1,
%    color=black,
%    contents={\begin{tikzpicture}[remember picture, overlay, font=\sffamily]
%       \node at ([xshift=3cm,yshift=1.5cm] current page.north east)
%             {\includegraphics[width = 2.5cm]{Phasecraft-HorizontalLogo.pdf}};
%      \node at ([xshift=3cm,yshift=-1.5cm] current page.north west)
%             {CONFIDENTIAL DRAFT};
%      \end{tikzpicture}}
%  }

\usepackage[
    backend=bibtex,
    style=numeric,
    sorting=none,
    maxnames=999, % This ensures that all author names are displayed
    minnames=1    % Minimum number of names before using "et al."
]{biblatex}
\bibliography{references}



%%%%%%%%%%%%%%%
%% Maths
%%%%%%%%%%%%%%%
\usepackage{amsmath}
\usepackage{braket}
\usepackage{physics}

%%%%%%%%%%%%%%%
%% Miscellaneous useful stuff
%%%%%%%%%%%%%%%
\usepackage{listings}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{amssymb}
\usepackage[ampersand]{easylist}
\usepackage{enumitem}
\usepackage{hyperref}
\hypersetup{
  colorlinks = true, %Colours links instead of ugly boxes
  linkcolor={blue!50!black}, %Colour of internal links
  citecolor=red, %{red!50!black}, %Colour of citations
  urlcolor=blue, %Colour for external hyperlinks
  linktoc=page,
}
\usepackage[capitalise, nameinlink]{cleveref}
\usepackage[
  style=long,
  nolist, 
  nonumberlist,
  nopostdot,
  acronym,
  toc=true, 
]{glossaries}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{multirow}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\usepackage{array}
\usepackage[british]{babel}
\usepackage{adjustbox}
\usepackage{comment}
%\usepackage{algorithm}
%\usepackage{algpseudocode}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\newcommand{\SubItem}[1]{
    {\setlength\itemindent{15pt} \item[-] #1}
}

